Conditional set generation using Seq2seq models

Conditional set generation learns a mapping from an input sequence of tokens to a set. Several NLP tasks, such as entity typing and dialogue emotion tagging, are instances of set generation. Seq2Seq models, a popular choice for set generation, treat a set as a sequence and do not fully leverage its key properties, namely order-invariance and cardinality. We propose a novel algorithm for effectively sampling informative orders over the combinatorial space of label orders. We jointly model the set cardinality and output by prepending the set size and taking advantage of the autoregressive factorization used by Seq2Seq models. Our method is a model-independent data augmentation approach that endows any Seq2Seq model with the signals of order-invariance and cardinality. Training a Seq2Seq model on this augmented data (without any additional annotations) gets an average relative improvement of 20% on four benchmark datasets across various models: BART, T5, and GPT-3. Code to use SETAUG available at: https://setgen.structgen.com.

==> colorcommands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{xspace}
\usepackage{ulem}
\definecolor{cosmiclatte}{rgb}{1.0, 0.97, 0.91}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0.4,1,0.2}
\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{0.9,0,0}
\definecolor{Orange}{rgb}{1,0.5,0}
\definecolor{yellow}{rgb}{0.65,0.6,0}
\definecolor{cadmiumgreen}{rgb}{0.2, 0.7, 0.24}


\newcommand{\squishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
\newcommand{\reallysquishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{0.2em} \setlength{\labelwidth}{0.2em}
      \setlength{\labelsep}{0.2em} } }

 \newcommand{\squishend}{
     \end{list} 
 }
% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}
\newcommand{\corr}[2]{\textbf{\textcolor{red}{\sout{#1} #2}}}
% \newcommand{\emnlpadd}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\red}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\aman}[1]{\textcolor{orange}{[#1 \textsc{--Aman}]}}
\newcommand{\dheeraj}[1]{\textcolor{blue}{[#1 \textsc{--Dheeraj}]}}
\newcommand{\antoine}[1]{\textcolor{red}{[#1 \textsc{--Antoine}]}}
\newcommand{\niket}[1]{\textcolor{red}{[#1 \textsc{--Niket}]}}
% \newcommand{\yy}[1]{\textcolor{red}{[#1 \textsc{--Yiming}]}}
\newcommand{\yy}[1]{}
% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}
\newcommand{\note}[1]{{\textcolor{purple}{[#1 \textsc{--note}]}}}


==> sections/backgroundrel.tex <==
\section{Background and related work}
\label{sec:background}
\paragraph{Notation}
Our focus is the setting where we are given a corpus $\train$ of $\{(\vx_i, \sY_i)\}_{i=1}^{m}$ where $\vx_i$ is a sequence of tokens and $\sY_i=\{\ry_1, \ry_2, \ldots, \ry_k\}$ is a set.
% \st{A popular example of such setting~(and the one we use for our experiments) is multi-label classification.} 
For example, in multi-label fine-grained sentiment classification, $\vx_i$ is paragraph and  $\sY_i$ is the a set of sentiments expressed by the paragraph.
We use $\ry_i$ to denote an output symbol, $[\ry_i, \ry_j, \ry_k]$ to denote an ordered sequence of symbols and $\{\ry_i, \ry_j, \ry_k\}$ to denote a set.

\subsection{Set generation using \sts model}

\paragraph{Task} Given a sample $\{(\vx_i, \sY_i)\}_{i=1}^{m}$, the task of conditional set generation is to efficiently estimate $\pcond{\sY_i}{\vx_i}$.

In this work, we adopt \sts models for the task. \sts models factorize $\pcond{\sY_i}{\vx_i}$ in an autoregressive fashion using the chain rule: 
\begin{align}
    \pcond{\sY_i}{\vx_i} &= \pcond{\ry_1, \ry_2, \ldots, \ry_k}{\vx_i} \nonumber \\
    &=\pcond{\ry_1}{\vx_i}\prod_{j=2}^{k}\pcond{\ry_j}{\vx_i, \ry_1\ldots\ry_{j-1}}
\end{align}

Where we have used the order $\sY = [\ry_1, \ry_2, \ldots, \ry_k]$ to factorize the joint distribution using chain rule.
\st{Crucially} If the labels were independent, any of the $k!$ orders can be used to factorize the same joint distribution.
Consider an example $(\vx, \sY = \{\ry_1, \ry_2\})$ pair.
By chain rule, we have the following equivalent factorizations of this sequence:
$\pcond{\sY}{\vx} = \pcond{\ry_1}{\vx}\pcond{\ry_2}{\vx, \ry_1} = \pcond{\ry_2}{\vx}\pcond{\ry_1}{\vx, \ry_2}$.
In theory, each of these orders ($[\ry_1, \ry_2]$ and $[\ry_2, \ry_1]$) is exchangeable, and should not affect the learning process.
In practice, however, the choice of order is important \dheeraj{why? give a reason here}.
\st{To the best of our knowledge, only} Prior work including \dheeraj{how about this rewrite? } \citet{vinyals2015order} have noticed this discrepancy between theory (order should not matter due to order invariance of the chain rule) and practice~(order of the output token matters for language modeling tasks) when using LSTM based \sts models. \dheeraj{I dont know if it's a discrepancy per se. The assumption theory makes is correct. The issues comes with ``choice" of label set and in real-world use-case, it can't be guaranteed to be independent all the time}
They have
\antoine{\citet{vinyals2015order} may have noticed it and modeled with it in mind, but I doubt they're the only ones to \textit{notice} this discrepancy}.






\subsection{Set generation in other settings}
Set generation has received considerable attention in the computer vision community.
Specifically, \citet{rezatofighi2018deep,rezatofighi2020learn} \st{were one of the first in the lines of work to} \dheeraj{Don't want to make claims like ``first", etc. If we missed something, it will greatly harm the paper} investigate set outputs for vision tasks.
Their learning procedure involves jointly learning  the order and the cardinality of the set.
However, their method relies on searching through a combinatorial space of permutations.
Our approach differs from their work in two important ways: i) instead of performing exhaustive search over the sample space, we add informative order over labels in the input, ii) we model cardinality simply by listing the set size as the first element of the sequence, and thus jointly learn both it with the set output.
\citet{nandwani2020neural} look at non-autoregressive approaches for set-generation. \dheeraj{seems incomplete, what did they do and how was it not enough to motivate the need for our work.. }
%and note that the problem might not arise in principle for autoregressive models. 
%\antoine{Not sure how this relates}

\citet{zhang2020set} explore the usage of energy-based models for set prediction. 
Their learning and inference procedure relies on drawing samples from the set distribution, which is prohibitively expensive for extremely high-dimensional spaces like text.

\citet{chen2021order} explored the generation of an optimal order for graph generation \textit{given} the nodes.
They observed that ordering nodes before inducing edges improves graph generation.
However, in our case, since the labels themselves are being generated, conditioning on the labels to create the optimal order is is not feasible.

Image classification and tagging typically involves a small, independent number of tags.
In contrast, \nlp tasks typically have label spaces spanning in thousands.
Our method is more suitable for such tasks as it does not rely on exhaustive search over label space and leverages label dependencies.

\paragraph{Specialized models for set generation}
\dheeraj{whats specialized models ? as opposed to ?}
A few methods have focused on developing specialized models to deal with set outputs.
These include using deep reinforcement learning~\cite{yang2019deep} for multi-label classification, and ~\cite{ye2021one2set} for extracting and generating keyphrases.
Different from these works, our focus is on methods that can optimally adapt \dheeraj{exisiting ?} \sts models for set generation.
\dheeraj{seems a little too claimy the following sentences, my suggestion is dropping it, rather we should emphasize the simplicity of our approach and how we don't need to retrain models from scratch again..}
The importance of our work is underscored by the near universality of \sts architectures. 
Large pre-trained models are becoming increasingly easier to use, and have continuously established the state of the art on a variety of problems that were earlier the prerogative of specialized models.
Thus, it is important to develop a deeper understanding of their properties in different settings.


\paragraph{Modeling set input}
Considerable work has looked at dealing with set-shaped inputs. 
Notably, \citet{zaheer2017deep} show that adding the input representations and feeding the resulting features to a non-linear network is a principled way of representing sets.

~\citet{murphy2019janossy} Also focused on the input encoding.

Add discussions from  \url{https://fabianfuchsml.github.io/learningonsets/} if relevant.

\dheeraj{Add a line at the end that we do output space, otherwise it looks awkwardly positioned}

==> sections/cardinality.tex <==
\section{Modeling cardinality}
\dheeraj{Too small a section, fold into previous section}

Let $m=|\sY|$ be the cardinality of $\sY$ (or the number of elements in $\sY$).
Our goal is to jointly estimate $m$ and $\sY$ (i.e., $\pcond{m, \sY}{\vx}$).
Additionally, the model should be able to use cardinality information for generating all the elements.
To this end, we simply add the order information at the beginning of the sequence. 
That is, we convert a sample $(\vx, \sY)$ to $(\vx, [|sY|, \pi(\sY)])$, and then train our \sts model as usual from $\vx \rightarrow [|sY|, \pi(\sY)]$.
Listing the order information ensures that the sequence factorizes as $\pcond{[|sY|, \pi(\sY)]}{\vx} = \pcond{|sY|}{\vx}\pcond{\pi(\sY)}{|sY|, \vx}$.
Thus, the generation of $\sY$ is conditioned on both the input and the cardinality as desired~(note the $\pcond{\pi(\sY)}{|sY|, \vx}$ term).

\paragraph{Why should cardinality help?}
\dheeraj{Maybe we should talk about how decoder attention now also has more information to attend to ? Not sure myself}
Unlike typical sequence generation problems where the number of tokens in the output do not follow a strict distribution, sets might have a fixed number of elements generated per input.
A model that learns the number of shapes to generate can thus avoid over-generation, a major problem with language generation models~\citep{welleck2019neural,fu2021theoretical}.


==> sections/commands.tex <==
\newcommand{\comet}{\textsc{comet}}
\newcommand{\bleu}{\textsc{bleu}}
\newcommand{\rouge}{\textsc{rouge}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> sections/intro-more-abstract.tex <==
\section{Introduction A}

% \note{Order, then cardinality. The rest of the paper follows this as well. Don't confuse order invariance with adding informatiNote that our approach enables us to use corpus-level statistics for making these decisions for fixingorders, an advantage that approaches that optimize thUnder review as a conference paper at ICLR 20224ADDING INFORMATIVE ORDERS FOR SET OUTPUTAs discussed in Section 3,SEQ2SEQformulation requires the output to be in a sequence.  Further,the order of the sequence is a crucial design choice that can drastically affect the performance. Priorwork (Vinyals et al., 2016; Rezatofighi et al., 2018; Chen et al., 2021) has noted that adding or-ders that have the highest conditional likelihood given the input is an optimal choice.  Specifically,(Vinyals et al., 2016; Rezatofighi et al., 2018) rely on exhaustive search over the space ofN!pos-sible orders during training,  and thus cannot scale to practical settings.  [isn’t this repeated fromprevious section?   –DHEERAJ] Chen et al. (2021) learn an optimal ordering over the nodes of agraph. However, their method relies on knowing the nodes beforehand. Different from these meth-ods, we sidestep exhaustive search and optimizing over optimal orders during training by proposingTSAMPLE, a novel method that tractably creates informative orders over sets. We augment data fromTSAMPLE, and the rest of the process proceeds asSEQ2SEQtraining.  [I think we should start fromhere for this section, the previous is repetitive from related work section –DHEERAJ]Our core insight is that knowing the optimal order between pairs of symbols in the output drasticallyreduces the possible number of permutations (by a factor of 2 for each constraint). We thus imposepairwise order constraints for a subset of labels.  Specfically, given an output set y1,y2,...,yk, ifyi,yj∈Yare independent, they can be added in an arbitrary order. Otherwise, an order constraintis added to the order between yi,yj.We   estimate  the   dependence  between   elements   yi,yjusing   pointwise  mutual   information:pmi(yi,yj)  =p(yi,yj)/p(yi)p(yj).   [Isn’t  there  a  log  component  in  PMI  ?  In  my  understand-ing, PMI was not a probability but this section seems to suggest so. I think I am missing somethinghere, not sure..  –DHEERAJ] Here,pmi(yi,yj)>1indicates that the labels yi,yjco-occur morethan would be expected under the conditions of independence (Wettler & Rapp, 1993) [not sure ifwe should explain PMI, I think the equation should suffice –DHEERAJ].  We usepmi(yi,yj)> αto  filter  our  such  pairs  of  dependent  pairs,  and  perform  another  check  to  determine  if  the  orderbetween  them  should  be  fixed.   For  each  dependent  pair  yi,yj,  the  order  is  constrained  to  be[yi,yj]iflogp(yj|yi)−logp(yi|yj)> β(yjshould come after yi),  and[yj,yi]otherwise.logp(yj|yi)−logp(yi|yj)> βimplies that knowledge that a set contains yi, increases theprobability of yjbeing present. Thus, fixing the order to[yi,yj]will aid the model in learning.The generality ofTSAMPLEis reinforced by noting two key properties of random variables [whyis generality reinforced ?  not sure I am getting the point about generality –DHEERAJ].  First, de-pendence between pair of variables is retained in joint distributions involving more variables (yi6⊥⊥yj=⇒yi6⊥⊥yj,yk) for someyk∈Y(Appendix A). Further, if yi,yj⊥⊥yk, then it can be shownthatp(yi|yj)> p(yj|yi)  =⇒p(yi|yj,yk)> p(yj|yi,yk)(Appendix D). The first propertyshows that the pairwise dependencies hold in presence of other elements of the set.  The secondproperty shows that independent symbols can be added to an informative order, and the resultinglonger sequence will continue to be informative.  Thus, our criteria of using pairwise dependenciesbetween the elements of a set is still effective.To systematically create permutations that satisfy these constraints, we construct a topological graphGwhere each node is a labelyi∈Y, and the edges are determined using the pmi and the conditionalprobabilities as outlined above (Algorithm 1).  The required permutations can then simply be gen-erated as topological traversalsG(Figure??).  To generate diverse samples, we begin the traversalfrom a different starting node.  We can see our method as an alternative proposal distributionqthatsamples from the topological graph. We call this methodTSAMPLE.[The following paragraph breaks the flow in a strong way..  We are in the process of describing ourmethod, we should not veer away to tell more stuff about how good our approach is.   –DHEERAJ]Note that our approach enables us to use corpus-level statistics for making these decisions for fixingorders, an advantage that approaches that optimize the order for each example do not enjoy [not sureI understand this line and not sure what the goal is –DHEERAJ].  Finally, restrictingTSAMPLEtopairwise dependencies helps with both scalability and correctness [how ?  Its a tall claim, we needto back it up or drop it –DHEERAJ]. Higher-order dependencies might not be accurately discovereddue to sparsity, and thus cause spurious orders [Not sure I understand this either –DHEERAJ].  Forsimilar reasons, we do not consider the inputXand only capture the dependence between the outputlabels [Same... Not sure I understand this either –DHEERAJ].e order for each example do not enjoy [not sureI understand this line and not sure what the goal is –DHEERAJ].  Finally, restrictingTSAMPLEtopairwise dependencies helps with both scalability and correctness [how ?  Its a tall claim, we needto back it up or drop it –DHEERAJ]. Higher-order dependencies might not be accurately discovereddue to sparsity, and thus cause spurious orders [Not sure I understand this either –DHEERAJ].  Forsimilar reasons, we do not consider the inputXand only capture the dependence between the outputlabels [Same... Not sure I understand this either –DHEERAJ]ve orders. These are two different things we are only doing latter!}
\aman{Dheeraj: please feel free to remove stuff from this intro that you don't need, like the para outlines later.}
Conditional set generation is the task of modeling the distribution of an output set given an input sequence of tokens.
Several natural language processing (\nlp) tasks are instances of set generation, including open-entity typing \dheeraj{add citation to each}, fine-grained emotion classification, and keyphrase generation.\aman{to think of it, all multi label classification tasks are an instance. we shouldn't restrict to just these/is there a better way of saying this?}
Recently, the sequence-to-sequence (\sts) framework has been successful for modeling structured output such as graphs \dheeraj{citation}, code and sets
in \nlp due to its simplicity and the ability to leverage the pretraining-finetuning paradigm. 


% Additionally, pretrained \sts models have recently shown state-of-the-art performance on structured output tasks - such as code and graph generation. \dheeraj{my suggestion is drop this line}
%, ---- which have traditionally been a prerogative of specialized models, underscoring the universal applicability of the \sts framework.

This paper argues that modeling set generation as a vanilla \sts generation task is sub-optimal as the \sts formulations do not model two key properties of a set output: \textit{order-invariance} and \textit{cardinality}.
Although prior work has highlighted the importance of modeling the order-invariant nature of both set inputs~\citep{zaheer2017deep} and outputs~\citep{vinyals2015order,rezatofighi2018deep}, effectively modeling them remains an open challenge.\footnote{Our work focuses on settings where the input is a sequence, and the output is a set.}

\begin{figure*}[!htb]
\centering
  \includegraphics[width=\linewidth]{img/main_fig.pdf}
\caption{The figure illustrates a sample task where given an input $\vx$, the output is a set of shapes.
Our method first learns a partial-order graph over the label space.
We use this structure to sample datapoints, which is then used to train the \sts model.
Additionally, we jointly model the cardinality by augmenting it as part of the set output (shown in the right).\aman{replaced}}
\label{fig:method}
\end{figure*}

Our paper addresses both these challenges. Figure \ref{fig:method2} shows our overall approach. Firstly, we propose an approach that imposes a partial-order graph on the label-space~(\ours), where the nodes are the labels and edges capture the dependency between nodes.
A training set sampled from this partial-order graph enforces better ordering of the labels compared to the original dataset for a \sts model. 
Interpreting the data creation process through variational inference, we show that \ours provides a better proposal distribution by leveraging the inherent ordering of the dataset label space. 
For cardinality, we propose a simple approach where we augment the cardinality as part of the output sequence. 
Together, we show that incorporating the properties of the set provides significant performance gains. 

Our experiments on three real-world diverse NLP datasets namely - XYZ show that we achieve better performance compared to baseline approaches. Specifically, we show that when the label space is large (\dheeraj{dataset name with some detail}), our approach is most effective. \dheeraj{I am debating to put theoretical statement here or in previous passage} We complement the empirical evaluation with theoretical discussion where we show that interpreting the data creation process of sequence to set as a variational inference problem, we show that our graph proposes a better proposal distribution. We also perform additional human analysis on the recovered order structures from dataset and interpret the nature of their dependencies. This result is significant as we show that through purely data augmentation approaches we can incorporate the properties of set in output space without making custom architectural or training changes to the model. 



\paragraph{Para 3/4: Our model leverages dependence between labels to add informative orders to the training data.}

\begin{enumerate}
    \item While set has no order, \sts requires one. The choice of order becomes crucial as certain orders might be more informative than the others.
    \item We leverage dependencies between set labels to find such informative orders.
    \item Specifically, our method arranges the labels in a partial-order graph where each node is a label, and edges constrain the order in which the labels appear.
    \item Our method enforces constraints between two labels if presence of one would help the generation of the other.
\end{enumerate}


\paragraph{Para 5: }
\begin{enumerate}
    \item For a given training dataset, the set output might have a few fixed sizes.
    \item Conditioning the generation on the set on its size has natural advantages.
    \item The model can avoid generating spurious labels, focus weights on the useful labels.
\end{enumerate}


To jointly model a set and its cardinality, we simply include the size of the set as the first element in the sequence. Due to auto-regressive factorization, the generation of the set is naturally conditioned on the predicted size.


% Further, we also propose a novel data augmentation strategy, \ours, which leverages the latent dependencies in the label space to generate more informative orderings of the set to maximize the task performance. 
% This is advantageous because it is more computationally tractable than augmenting the data with all the set permutations (mainly when the label space is ample). 



Empirically, we establish the utility and soundness of our approach by showing gains in three real-world \nlp datasets~($\sim$10\% gains in both micro and macro f-scores).
This result is significant - we effectively show that simple techniques such as augmenting cardinality and automated data augmentation approaches can substantially improve sequence to set generation tasks without any additional annotation overhead.
We also provide a theoretical grounding for our approach -- treating the order as a latent variable, we show that \ours serves as a better proposal distribution in a variational inference framework.
Finally, we perform an in-depth analysis of the reasons behind the sensitivity of the \sts framework on order by experimenting with a graphical model that realistically mimics a conditional set generation setting. 


\paragraph{Our contributions}
(i) we show an efficient way to model sequence-to-set prediction as an \sts task by jointly modeling the cardinality and proposing a novel \ours data augmentation approach to add informative sequences. (ii) we show theoretically and empirically that our approach is better suited for set generation tasks than existing approaches. 
(iii) we also perform an in-depth analysis, providing several avenues for future research. \aman{tighten this}

==> sections/introduction.tex <==
\section{Introduction v1.0}


\paragraph{TL; DR} We propose an efficient and effective way to do set-generation as \sts task. We leverage key properties of a set, namely cardinality and order-invariance, for effective set generation within the \sts framework. \corr{before}{suggested change}

% \paragraph{\sts models have become popular.}
% \begin{enumerate}
%     \item What is set generation?
%     \item Why should we use \sts models for it, why not specialized models? Why is \sts so attractive?
%     \item What has been done, what is the gap?
%     \item Contributions.
% \end{enumerate}

Conditional set generation is the task of modeling the distribution of an output set given (conditioned on) an input sequence of tokens.
Several popular natural language processing (\nlp) tasks are instances of set generation, including open-entity typing, fine-grained emotion classification, and keyphrase generation~(Figure~TODO).


Recently, the sequence-to-sequence (\sts) framework has become an attractive choice for modeling set generation problems in \nlp{} due to its simplicity and the ability to leverage the pretraining-finetuning paradigm \citep{yang2018sgm}. 
% There are several reasons for this popularity.
% First, adapting set generation as a \sts modeling task is relatively straightforward: the set can simply be flattened as a sequence.
% Notably, as \sts modeling uses auto-regressive factorization~(chain rule), the output can be listed in any order \textit{in principle}.
Additionally, pretrained \sts models have recently shown state-of-the-art performance on tasks with a sequence as an input and a structured output - such as code and graph generation. \antoine{Is this relevant to set generation?} \aman{During informal discussions a lot of people ask: why do you event want to do \sts for set generation? This paragraph is \textit{supposed} to address that concern.} \dheeraj{I also feel this line can be dropped}
%, ---- which have traditionally been a prerogative of specialized models, underscoring the universal applicability of the \sts framework.



This paper argues that treating set generation as a vanilla \sts generation task is sub-optimal as the current \sts formulation does not explicitly model two key properties of a set output: \textit{cardinality} \st{(the number of elements)} \dheeraj{weird to explain one and not other}, and \textit{order-invariance}.
Although prior work has highlighted the importance of modeling the order-invariant nature of both set inputs~\citep{zaheer2017deep} and outputs~\citep{vinyals2015order,rezatofighi2018deep}, modeling them effectively remains an open challenge. \dheeraj{if we are focusing only on output, shouldn't we talk about output alone ? It will sound like bait-and-switch otherwise}
\footnote{Our work focuses on settings where the input is a sequence, and the output is a set.}

\paragraph{Why are these two properties useful?}
\begin{enumerate}
    \item Order 
\end{enumerate}


We propose a novel method, \ours, to effectively model set-generation as a \sts task. 
Our method accounts for the intrinsic properties of a set - namely, the cardinality and the order-invariance. \aman{repeated?} \antoine{yes}
To make the model order invariant, we propose a novel data augmentation strategy, \ours, which exploits dependencies between labels to generate an informative ordering of the set. \antoine{you mention cardinality first as a problem, but described a solution to order-invariance first. It's better to remain consistent}
The set is listed as a sequence, but several carefully selected permutations of the same set are added to the training data \antoine{define "carefully selected" -- is it manual? if not, give more description}. 
This allows the model to learn the order invariant nature of the set output while leveraging the conditional dependence relations between the labels. \antoine{this make sit sound as though ``leveraging the conditional dependence relations'' is an unexpected byproduct. In fact, it's the motivation of your method -- I'd rewrite this paragraph from a more proactive perspective. }
To jointly model a set and its cardinality, we simply include the size of the set as the first element in the sequence.
% Further, we also propose a novel data augmentation strategy, \ours, which leverages the latent dependencies in the label space to generate more informative orderings of the set to maximize the task performance. 
% This is advantageous because it is more computationally tractable than augmenting the data with all the permutations of a set (mainly when the label space is ample). 

\begin{figure*}[!htb]
\centering
  \includegraphics[width=\linewidth]{img/main_fig.pdf}
\caption{Given a corpus of input-set output pairs~(left), a partial order graph over the labels (middle) is used to generate informative orders over the set of labels. 
The orders are used to serialize sets into sequences. 
The figure illustrates a sample task where given an input $\vx$, the output is a set of shapes~(\eg pyramid, quadrilateral, triangle). The partial order graph arranges the label space such that specific labels~(dodecahedron, pyramid) come before more general labels~(square, triangle).
During learning and inference, listing the specific labels first gives the model more clues about the rest of the set, leading to more informative sequences.
The size of each set is also added as the first element for joint modeling of output with size.
}
\label{fig:method2}
\end{figure*}

We establish both theoretically and empirically why our proposed approach achieves the performance gains. \antoine{before talking about ``why,'' you need to establish that you get performance gains in the first place}
We show that \ours serves as a better proposal distribution in a variational inference framework with the order as a latent variable, which helps in effectively sampling informative orders \antoine{put at end. this sounds like an unexpected result. if it's not, you should describe in a prior paragraph WHY that you were trying to accomplish this result}.
Empirically, we show substantial gains in three real-world NLP datasets with large label spaces compared to existing approaches that model set generation as a \sts task. This result is significant - we effectively show that simple techniques such as augmenting cardinality and automated data augmentation approaches can substantially improve sequence to set generation tasks without any additional annotation overhead.

\paragraph{Our contributions}
(i) we show an efficient way to model sequence-to-set prediction as an \sts task by jointly modeling the cardinality and proposing a novel \ours data augmentation approach to incorporate the order-invariant nature of the set. (ii) we show theoretically and empirically that our approach is better suited for set generation tasks than existing approaches. 
(iii) we also perform an in-depth analysis, providing several avenues for future research. 



% We show that jointly modeling set output with its cardinality and augmenting training data with random orders can improve the performance substantially \dheeraj{I thought this was already prior work, why are we showing this again ?}.
% We then propose a novel data augmentation strategy, \ours, that helps sample more informative orders from the combinatorial space.
% We also show that \ours and existing strategies can be generalized by a variational inference framework, giving theoretical grounding to the advantages offered by our approach.
% We show the utility of our approach and analysis by thorough experiments on a graphical model that realistically mimics a conditional set generation setting.
% Additionally, we show that our approach benefits three diverse set-generation datasets.
% This result is important, since the simplicity of the approach can be easily adapted across many tasks. 
% We identify a large class of \nlp tasks as a set generation problem and propose a solution.
% that \ours and existing strategies can be generalized by a variational inference framework, giving theoretical grounding to the advantages offered by our approach.
% We show the utility of our approach and analysis by thorough experiments on a graphical model that realistically mimics a conditional set generation setting.
% Additionally, we show that our approach benefits three diverse set-generation datasets.
% This result is important, since the simplicity of the approach can be easily adapted across many tasks.
%that helps in sampling more informative orders of the label space which
% from the combinatorial space.
% First, the behavior of modern transformer-based \sts models for set generation is unknown, as prior work has exclusively focused on \lstm based models.
% Further, efficient solutions for real-world \nlp use cases have not been explored, as the role of order has only been studied in a simulation setting or for uses cases with a relatively small output space.
% Finally, prior studies did not closely examine the reasons for the role of order and in set generation and have motivated the problem and solution only with empirical evidence.

==> sections/introv3.tex <==
\section{Introduction}
\yy{Maybe just call the task multi-label generation. Set generation implies that the output set is independent. If you just say multi-label prediction, you cover both the cases. Set generation is not the right word. The point of using a graph is that there is some label dependency. Use the problem into multi-label generation. Argue what kind of data sources can be used for generating. You define the space of shapes, and multi-level; it's not something you learn from the data (you discover it). Keep including examples from multi-label prediction in this problem. Wikipedia graph could be another source of this hierarchy (in other words, instead of instantiating the whole graph, you need some passes). It might also be a good idea to compare your approach when you have pre-existing. You need some trade-off it cannot be a sequence, it cannot be a set, it has to be in the middle. Defining the problem as set prediction is equally wrong.}

\yy{A language is somewhere in the middle: it is neither all disjoint nor everything is in order. There are certain orders that appear more often. We are not ordering either of the extremes. Some elements of the elements we have are independent, and the others are not. 
That is why there is room for the topological graphs.
If the output was just set of independent elements. If the output was just a set of independent elements, you can sample from uniform.
}
% \note{Order, then cardinality. The rest of the paper follows this as well. Don't confuse order invariance with adding informative orders. These are two different things we are only doing latter!}


% \niket{table of assumptions checkpointing with each dataset and also list datasets where this will not work (scope)}

% \niket{apply your method atleast in principle on openpi dataset}

% \niket{the small result on set size (thinking about the answer) .. but it also works for list}

% \niket{you should add some more related work.}

% \niket{placing your work -- order matters 2016 paper -- surprising for very large models. perhaps show T5-XXL. larger models memorize the input patterns.}


% https://www.semanticscholar.org/paper/Seq-SetNet%3A-Exploring-Sequence-Sets-for-Inferring-Ju-Zhu/18a4f953e306210827f6251263071480b105c66f

Conditional set generation is the task of modeling the distribution of an output set given an input sequence of tokens~\citep{kosiorek2020conditional}.
Several natural language processing (\nlp) tasks are instances of set generation, including open-entity typing~\citep{choi2018ultra,dai2021ultra} and fine-grained emotion classification~\citep{demszky2020goemotions}.
The recent successes of pretraining-finetuning paradigm have encouraged a formulation of set generation as a sequence-to-sequence~(\sts) generation task~\citep{vinyals2015order,yang2018sgm,meng2019doesordermatter,ju2020transformer}.
%, due to its simplicity and the ability to leverage the sequence-to-sequence (\sts) framework.
% Recently, the sequence-to-sequence (\sts) framework has been successful for modeling structured output such as graphs \dheeraj{citation}, code and sets in \nlp due to its simplicity and the ability to leverage the pretraining-finetuning paradigm.


In this paper, we posit that modeling set generation as a vanilla \sts generation task is sub-optimal, because the \sts formulations do not explicitly account for two key properties of a set output: \textit{order-invariance} and \textit{cardinality}. 
Forgoing order-invariance, vanilla \sts generation modeling treats a set as a sequence, assuming an arbitrary order between the elements it outputs. 
%Similarly, the cardinality of sets is typically not explicitly modeled. 
Similarly, the cardinality of sets is ignored, as the number of elements to be generated is typically not explicitly modeled.

Prior work has highlighted the importance of these two properties 
% \corr{for modeling set-shaped input~\citep{zaheer2017deep,santoro2017simple,huangbetter2020,kim2021setvae} and} ~\citep{vinyals2015order,rezatofighi2018deep,qin2019adapting}
for set output through loss functions that encourage order invariance~\citep{ye2021one2set}, exhaustive search over the label space for finding an optimal order~\citep{qin2019adapting,rezatofighi2018deep,vinyals2015order}, and post-processing the output~\citep{chowdhury2016know2look}.
%typically perform exhaustive search over the label space. either rely on making architectural changes to the model or performing an exhaustive 
Despite the progress, several important gaps remain to be addressed.
First, exhaustive search does not scale with large output spaces typically found in \nlp problems, thus stressing the need for an optimal sampling strategy for the labels. % \corr{Second, overgeneration has long been recognized as a problem in conditional text generation in \sts settings~\citep{xie_neural_nodate,moryossef_step-by-step_2019}}{}.
%the promising solution of modeling output cardinality has received little attention. 
Second, despite being an essential aspect for a set, cardinality is still not explicitly modeled in \sts setting.
Finally, architectural modifications required to use specialized set-generation techniques might not be viable for modern large-language models.
%, and thus cannot be used out of box/which might not be possible in case of large pre-trained language models.

% \squishlist
% \item Exhaustive search: 
% \item jointly modeling cardinality: 
% \item Architectural modifications (loss functions, specialized modules): 
% \squishend


\begin{figure*}[!t]
\centering
  \includegraphics[scale=0.20]{img/main_fig_v14.pdf}
\caption{
An illustrative task where given an input $\vx$, the output is a set of emotions. 
Our method first discovers a partial order graph~(middle) in which specific labels~(joy) come before more general labels~(pride).
Listing the specific labels first gives the model more clues about the rest of the set.
Topological samples from this partial order graph yield label sequences that are more efficiently generated using \sts models.
The size of each set is also added as the first element for joint modeling of output with size.}
\label{fig:method}
\end{figure*}


We address these challenges with a novel data augmentation strategy.
%\niket{it sounds like past work has not used \sts? what about work with RNNs \cite{meng2019doesordermatter}}, the question of effectively modeling set output using \sts models still remains an open challenge \niket{should we mention training infeasibility with very large models gpt3 lambda etc.?} .\footnote{Our work focuses on settings where the input is a sequence, and the output is a set.}
%\red{Further, the ever increasing size}
%\textbf{1. Exhaustive search, 2. cardinality  3. Training infeasibility}
%Listing the set as a sequence in an arbitrary order might ignore such dependencies that could otherwise be leveraged for an effective generation.
% Our method addresses the challenges above by taking 
Specifically, we take advantage of the auto-regressive factorization used by \sts models and (i) impose an \textit{informative} order over the label space, and (ii) explicitly model \textit{cardinality}. First, the label sets are converted to sequences using informative orders by grouping labels and leveraging their dependency structure. 
%A natural way to model this is to search exhaustively for the best label orders. 
To efficiently search for such informative orders over a combinatorial space, our method imposes a partial order graph over the labels, where the nodes are the labels and the edges denote the conditional dependence relations.
% The nodes of the partial order graph are the labels, and the edges reflect pairwise constraints for labels in the sequence. 
We then generate the training data with orders over the label set that are sampled by performing topological traversals over the graph.
Labels that are not constrained by dependency relations are augmented in different positions in each sample, reinforcing the order-invariance. We then create an augmented training dataset, where each input instance is paired with various valid label sequences sampled from the dependency graph. 
Next, we jointly model a set with its cardinality by simply prepending the set size to the output sequence.  
This strategy also aligns with the current trend of very large language models which do not lend themselves to architectural modifications, but increasingly rely on informativeness of the inputs~\citep{yang2020g,Liu2021PretrainPA}.

% Further, unlike sequence output, the distribution of the set output size~($\pcond{|\sY|}{\vx}$) might have a few modes and can give useful information for set generation.



\Figref{fig:method} illustrates the key intuitions behind our method using sample task where given an input $\vx$ (say a conversation), the output is a set of emotions~($\sY$).
To see why certain orders might be more meaningful, consider a case where one of the emotions is \textit{joy}, which leads to a more general emotion of \textit{pride}.
After first generating \textit{joy} a the drink, the model can generate \textit{pride} with certainty~(\textit{joy} leads to \textit{pride} in all samples).
In contrast, the reverse order (generating \textit{pride} first) still leaves room for multiple possible emotions~(joy and iced love).
The order $[\text{joy}, \text{pride}]$ is thus more informative than $[\text{pride}, \text{joy}]$.
% Similarly, there are cases where the shapes have no dependence, and can appear in any order.
% In such cases, listing the labels in any order will alleviate sparsity and induce the inductive bias of order invariance.
The cardinality of a set can also be helpful.
In our example, joy contains two sub-emotions, and love contains one.
A model that first predicts the number of sub-emotions can be more precise in its output and avoid over-generation, a major challenge with language generation models~\citep{welleck2019neural,fu2021theoretical}.
Our approach provides an efficient way of sampling such informative orders from the combinatorial space of all possible orders and jointly modeling cardinality by leveraging auto-regressive nature of \sts models.
% Further, we also propose a novel data augmentation strategy, \ours, which leverages the latent dependencies in the label space to generate more informative orderings of the set to maximize the task performance. 
% This is advantageous because it is more computationally tractable than augmenting the data with all the set permutations (mainly when the label space is ample). 
%Empirically, we establish the utility and soundness of our approach by showing performance improvements with a diverse set of \sts models on four real-world \nlp datasets ~($\sim$20\% relative improvement in \fs scores). 
%This result is significant - we effectively show that simple techniques such as augmenting cardinality and automated data augmentation approaches can substantially improve sequence to set generation tasks without any additional annotation overhead or architecture changes.
%Finally, we perform an in-depth analysis of the reasons behind the sensitivity of the \sts framework on order by experimenting with a simulated experiment that realistically mimics a conditional set generation setting. 
% \vspace{-3.3em}
\paragraph{Our contributions}
\squishlist
 \item[(i)] We show an efficient way to model sequence-to-set prediction as a \sts task by jointly modeling the cardinality and augmenting the training data with informative sequences using our novel \ours data augmentation approach.~(Section \ref{sec:tsample}, \ref{sec:modelingcardinality}).
\item[(ii)] We provide a theoretical grounding for our approach. Treating the order as a latent variable, \ours serves as a better proposal distribution when viewed via a variational inference framework.~(\Secref{par:vi})
%We theoretically justify our approach by treating the order as a latent variable and showing that our method derives orders from from an informative proposal distribution.
\item[(iii)] We show a $\sim$20\% relative improvement of \sts models, across four real world tasks, without any additional annotations or architecture changes.~(\Secref{sec:experiments}).
\squishend
% (iii) we also perform an in-depth analysis, providing several avenues for future research. \aman{tighten this}



==> sections/simulation_complete.tex <==
\section{Exploring the influence of order on \sts models with a simulation}
\label{sec:simulationcomplete}
We design a simulation to investigate the effects of output order and cardinality on conditional set generation, following prior work that has found simulation to be an effective for studying properties of deep neural networks~\citep{vinyals2015order,khandelwal2018sharp}.



\paragraph{Data generation}
We use a graphical model~(\Figref{fig:gmodelappendix}) to generate conditionally dependent pairs $(\vx, \sY)$, with different levels of interdependencies among the labels in $\sY$.
Let $\sY = \{\ry_1, \ry_2, \ldots, \ry_N\}$ be the set of output labels.
We sample a dataset of the form $\{(\vx, \vy)\}_{i=1}^{m}$.
$\vx$ is an $N$ dimensional multinomial sampled from a dirichlet parameterized by $\alpha$, and $\vy$ is a sequence of symbols with each $\evy_i \in \sY$.
The output sequence $\vy$ is created in $B$ \textit{blocks}, each block of size $k$.
A block is created by first sampling $k-1$ prefix symbols independently from $\text{Multinomial}(\vx)$, denoted by $\vy_{p}$
The $k^{th}$ suffix symbol ($y_{s}$) is sampled from either a uniform distribution with a probability = $\epsilon$ or is deterministically determined from the preceding $k-1$ prefix terms.
% Note that a block of size $k$ has $k-1$ prefix symbols independently sampled from $\textnormal{Multinomial}(\vp)$, whereas the last term depends on the prefix. 
For block size of 1 ($k=1$), the output is simply a set of size $B$ sampled from $\vx$ (i.e., all the elements are independent). 
Similarly, $k=2$ simulates a situation with a high degree of dependence: each block is of size 2, with the prefix sampled independently from the input, and the suffix determined deterministically from the prefix.
Gradually increasing the block size increases the number of independent elements.
%and $k=3$ simulate a unigram and bigram dependency, respectively.



% \begin{tabular}{cc}
% \raisebox{.1cm}{\begin{minipage}{.5\textwidth}
\begin{figure}[H]
  \centering
  \tikz{ %
    \node[obs] (alpha) {Dir($\alpha$)} ; %
    \node[latent, right=of alpha] (x) {$X$} ; %
    \node[latent, right=of x] (ypre) {$y_{p}$} ; %
    \node[latent, right=of ypre] (ysuff) {$y_{s}$} ; %
    \plate[inner sep=0.2cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(ypre)} {k-1}; %
    \plate[inner sep=0.2cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(ypre) (ysuff) (plate1)} {B}; %
    \plate[inner sep=0.2cm, xshift=-0.12cm, yshift=0.12cm] {plate3} {(x) (plate1) (plate2)} {M}; %
    \edge {alpha} {x} ; %
    \edge {x} {ypre} ; %
    \edge {ypre} {ysuff} ; %
  }
 \caption{The generative process for simulation}
 \label{fig:gmodelappendix}
\end{figure}
% \end{minipage}} &
% \begin{minipage}{.5\textwidth}
\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.4]{img/setgen_order_matters.pdf}
    \caption{Perplexity vs. Randomness for varying block sizes. The degree of dependence between the labels is highest for block size = 2, where each label depends the preceding label. In such cases, the model is most affected by shuffling the order at test time. In contrast, with block size of 1, the perplexity is nearly unaffected by the order. This result complements Lemma~\ref{sec:ordershouldnotmatter} in showing that order will not affect \sts models if all the labels are independent of each other.}
    \label{fig:pplvsorderappendix}
\end{figure*}

% \end{minipage}
% \end{tabular}


\subsection{Major Findings}

We now outline our findings from the simulation.
We use the architecture of \bart-base~\cite{lewis2020bart}~(six-layers of encoder and decoder) without pre-training for all simulations.
All the simulations were repeated using three different random seeds, and we report the averages.
\paragraph{Finding 1: \sts models are sensitive to order, but only if the labels are conditionally dependent on each other.}
We train with the prefix $\vy_p$ listed in the lexicographic order. 
At test time, the order of is randomized from 0\% (same order as training) to 100 (appendixly shuffled).
As can be seen from~\Figref{fig:pplvsorderappendix} the perplexity gradually increases with the degree of randomness.
% Crucially, note that the output was a randomly ordered set of symbols, with only the prefixes listed in the sorted order. Despite that, the model is sensitive to order.
Further, note that perplexity is an artifact of the model and is independent of the sampling strategy used, showing that order affects learning.



\paragraph{Finding 2: Training with random orders makes the model less sensitive to order}

As \Figref{fig:pplorderhelpsappendix} shows, augmenting with random order makes the model less sensitive to order.
Further, augmenting with random order keeps helping as the perplexity gradually falls, and the drop shows no signs of flattening.

%Finally, note that the drop in perplexity is gradual and shows no signs of slowing down. This concurs with our observation made in \Secref{sec:roleorder} that a primary cause of order dependence is lack of support.

\paragraph{Finding 3: Effects of position embeddings can be overcome by augmenting with a sufficient number of random samples}
\Figref{fig:pplorderhelpsappendix} shows that while disabling position embedding helps the baseline, similar effects are soon achieved by increasing the random order.
This shows that disabling position embeddings can indeed alleviate some concerns about the order.
This is crucial for pre-trained models, for which position embeddings cannot be ignored.

\begin{figure*}[!htb]
  \includegraphics[width=\linewidth]{img/setgen_order_helps.pdf}
\caption{Augmenting dataset with multiple orders help across block sizes. Augmentations also overcome any benefit that is obtained by using position embeddings.}
\label{fig:pplorderhelpsappendix}
\end{figure*}

\paragraph{Finding 4: \ours leads to higher set overlap} We next consider blocks of order 2 where the prefix symbol $\ry_p$ is selected randomly as before, but the suffix is set to a special character $\ry_p'$ with 50\% probability.
As the special symbol $\ry_p'$ only occurs with $\ry_p$, there is a high pmi between each $(\ry_p, \ry_p')$ pair as $\pcond{\ry_p}{\ry_p'} = 1$.
Different from finding 1, the output symbols are now shuffled to mimic a realistic setup.
We gradually augment the training data with random and topological orders and evaluate the learning and the final set overlap using training perplexity and Jaccard score, respectively.
The results are shown in \Figref{fig:toposetoverlapandpplappendix}.
Similar trends hold for larger block sizes, and the results are included in the Appendix in the interest of space.
% Further, note that there needs to be no correlation between set overlap and perplexity.
% Set overlap captures the ability of the model to sample more informative sequences, whereas perplexity captures the ability of the model to be sensitive to order.


\begin{figure*}[!htb]
  \includegraphics[width=\linewidth]{img/setgen_topo_ppl_set_overlap.pdf}
\caption{Effect of \ours on perplexity and set overlap. \textbf{Left:} Augmentations done \ours helps the model converge faster and to a lower perplexity. \textbf{Right:} Using \ours, the overlap between training and test set increases consistently, while consistently outperforming \rand.}
\label{fig:toposetoverlapandpplappendix}
\end{figure*}


\paragraph{Finding 5: \ours helps across all sampling types} We see from Table~\ref{tab:samplingtypesetoverlapappendix} that our approach is not sensitive to the sampling type used. Across five different sampling types, augmenting with topological orders yields significant gains.

\paragraph{Finding 6: \sts models can learn cardinality and use it for better decoding}

We created sample data from ~\Figref{fig:gmodelappendix} where the length of the output is determined by sum of the inputs $X$.
We experimented with and without including cardinality as the first element.
We found that training with cardinality increases step overlap by over 13\%, from 40.54 to 46.13.
Further, the version with cardinality accurately generated sets which had the same length as the target 70.64\% of the times, as opposed to 27.45\% for the version without cardinality.

\begin{table*}[]
\centering
\begin{tabular}{lrrrrr}
\toprule
         & Beam          & Random        & Greedy        & Top-k        & Nucleus    \\ \midrule
\rand  & $0.39\pm0.05$ & $0.39\pm0.02$ & $0.35\pm0.05$ & $0.39\pm0.02$ & $0.39\pm0.02$ \\
\ours & $0.67\pm0.05$ & $0.67\pm0.05$ & $0.71\pm0.04$ & $0.67\pm0.05$ & $0.68\pm0.05$ \\ \bottomrule
\end{tabular}
\caption{Set overlap for different sampling types with 200\% augmentations. The gains are consistent across sampling types. Similar trends were observed for 100\% augmentation and without positional embeddings. Top-k sampling was introduced by \citep{fan2018hierarchical}, and Nucleus sampling by \citep{holtzman2019curious}.}
\label{tab:samplingtypesetoverlapappendix}
\end{table*} 

